A Ferroelectric Compute-in-Memory Annealer for Combinatorial Optimization Problems

Computationally hard combinatorial optimization problems (COPs) are ubiquitous in many applications, including logistical planning, resource allocation, chip design, drug explorations, and more. Due to their critical significance and the inability of conventional hardware in efficiently handling scaled COPs, there is a growing interest in developing computing hardware tailored specifically for COPs, including digital annealers, dynamical Ising machines, and quantum/photonic systems. However, significant hurdles still remain, such as the memory access issue, the system scalability and restricted applicability to certain types of COPs, and VLSI-incompatibility, respectively. Here, a ferroelectric field effect transistor (FeFET) based compute-in-memory (CiM) annealer is proposed. After converting COPs into quadratic unconstrained binary optimization (QUBO) formulations, a hardware-algorithm co-design is conducted, yielding an energy-efficient, versatile, and scalable hardware for COPs. To accelerate the core vector-matrix-vector (VMV) multiplication of QUBO formulations, a FeFET based CiM array is exploited, which can accelerate the intended operation in-situ due to its unique three-terminal structure. In particular, a lossless compression technique is proposed to prune typically sparse QUBO matrix to reduce hardware cost. Furthermore, a multi-epoch simulated annealing (MESA) algorithm is proposed to replace conventional simulated annealing for its faster convergence and better solution quality. The effectiveness of the proposed techniques is validated through the utilization of developed chip prototypes for successfully solving graph coloring problem, indicating great promise of FeFET CiM annealer in solving general COPs.

==> 08_cover_letter.tex <==




Dear Editors and Reviewers,

Please find the enclosed manuscript entitled \textbf{"A Ferroelectric Compute-in-Memory  Annealer for Combinatorial Optimization Problems"}, which we wish to be considered for publication in Nature Electronics.

Our paper presents a novel hardware-algorithm co-design approach for a compute-in-memory (CiM) annealer, designed to efficiently address quadratic unconstrained binary optimization (QUBO) formulations of combinatorial optimization problems (COPs).
%It is widely recognized that many COPs, including graph coloring, the Max-Cut problem, and traveling salesman problem, etc., can be effectively reformulated as Ising spin glass models or QUBO formulations, which have emerged as power frameworks for solving these COPs. 
While various computing hardware solutions have been proposed to tackle COPs, they each come with their own limitations.
%by effectively implementing Ising model or QUBO formulations. 
Digital annealers, for instance,  compute the energy of the objective function  and employ advanced annealing algorithms to  locate the energy minima. However, their efficiency is hindered by the significant energy consumption and time delays associated with
%are energy- and time-consuming due to  
data movement between memory and computing units. 
Dynamical system Ising machines, on the other hand, leverage the inherent dynamics of the system  to 
%settle at ground energy state to 
naturally explore  solution spaces and identify spin combination that solves COPs.
Despite their advantages, these solvers still grapple with challenges related to  robustness,  scalability and  applicability to a wide range of COPs, primarily due to issues such as  sensitivity to accurate mapping of spin coupling terms, limitations in solving large-scale problems, and the  integration of self-interactions into solvers.

To overcome the limitations of existing computing hardware solutions,  our work proposes a compute-in-memory (CiM) annealers with several contributions: 
1) We pioneer the utilization of a ferroelectric field effect transistor (FeFET) based CiM array to accelerate the core QUBO computations, i.e., vector-matrix-vector (VMV) multiplications.
This is achieved by exploiting the distinctive three-terminal structure and nonvolatile memory (NVM) properties of FeFETs.
The FeFET crossbar stores
QUBO coupling  matrix elements, while two input vectors are applied to the FeFET gates and drains, respectively, for in-situ VMV multiplications;
2) 
Leveraging the  FeFET based CiM array's capacity to accelerate  VMV multiplications with asymmetric input vectors, we present a lossless QUBO matrix compression method. This technique significantly reduces  CiM array overhead, thereby increasing the problem-solving capacity for larger scale COPs;
3) We introduce the multi-epoch simulated annealing algorithm (MESA),  a novel approach that achieves optimal COP solutions through iterative QUBO computations within shorter time periods;
4) We demonstrate the first experimental prototypes of  FeFET CiM arrays to showcase its efficacy in accelerating QUBO computations and highly competitive performance compared to other hardware alternatives when solving complex COPs.

%In summary, our work proposes a FeFET based CiM annealer along with its matrix compression technique and the MESA process. Together, these approaches provide a promising hardware-algorithm co-design  platform for efficiently solving complex COPs.

Therefore, we believe that our work represents a significant advancement in developing appropriate hardware for solving COPs. We sincerely appreciate your consideration of our manuscript and look forward to valuable insights and comments from the esteemed reviewers. 

Sincerely, 

Xunzhao Yin, Thomas K{\"a}mpfe and Kai Ni
%Our contributions for the FeFET based CiM annealer approach for efficient COP solving include: 1) the first work on employing 1FeFET1R crossbar array for in-situ VMV multiplication acceleration 
